Semantics of Division for Polynomial Solvers

How to handle division in systems that compute with logical formulas involving what would otherwise be polynomial constraints over the real numbers is a surprisingly difficult question. This paper argues that existing approaches from both the computer algebra and computational logic communities are unsatisfactory for systems that consider the satisfiability of formulas with quantifiers or that perform quantifier elimination. To address this, we propose the notion of the fair-satisfiability of a formula, use it to characterize formulas with divisions that are well-defined, meaning that they adequately guard divisions against division by zero, and provide a translation algorithm that converts a formula with divisions into a purely polynomial formula that is satisfiable if and only if the original formula is fair-satisfiable. This provides a semantics for division with some nice properties, which we describe and prove in the paper.

==> ex1 <==

Consider input:  ex x[ z^2 - 3 x + 2 y^2 = 1 /\ y + y/x^2 <= 1 - (1/8) (z + y + 1)^2

> (def F [ex x [ z^2 - 3 x + 2 y^2 = 1 /\ [ x /= 0 /\ x^2 y + y <= x^2 - x^2 (1/8) (z + y + 1)^2]]])
:void
> F
ex x[z^2 + 2 y^2 - 3 x - 1 = 0 /\ x /= 0 /\ x^2 z^2 + 2 x^2 y z + 2 x^2 z + x^2 y^2 + 10 x^2 y + 8 y - 7 x^2 <= 0]:tar
> (qfr F)
[z^2 + 2 y^2 - 1 /= 0 /\ z^6 + 2 y z^5 + 2 z^5 + 5 y^2 z^4 + 10 y z^4 - 9 z^4 + 8 y^3 z^3 + 8 y^2 z^3 - 4 y z^3 - 4 z^3 + 8 y^4 z^2 + 40 y^3 z^2 - 34 y^2 z^2 - 20 y z^2 + 15 z^2 + 8 y^5 z + 8 y^4 z - 8 y^3 z - 8 y^2 z + 2 y z + 2 z + 4 y^6 + 40 y^5 - 32 y^4 - 40 y^3 + 29 y^2 + 82 y - 7 <= 0]:tar
> (def G [ex x [ z^2 - 3 x + 2 y^2 = 1 /\ [ x = 0 /\ y <= 1 - (1/8) (z + y + 1)^2]]])
:void
> (qfr G)
[z^2 + 2 y^2 - 1 = 0 /\ z^2 + 2 y z + 2 z + y^2 + 10 y - 7 <= 0]:tar

# the first part
(plot2d [z^2 + 2 y^2 - 1 /= 0 /\ z^6 + 2 y z^5 + 2 z^5 + 5 y^2 z^4 + 10 y z^4 - 9 z^4 + 8 y^3 z^3 + 8 y^2 z^3 - 4 y z^3 - 4 z^3 + 8 y^4 z^2 + 40 y^3 z^2 - 34 y^2 z^2 - 20 y z^2 + 15 z^2
 + 8 y^5 z + 8 y^4 z - 8 y^3 z - 8 y^2 z + 2 y z + 2 z + 4 y^6 + 40 y^5 - 32 y^4 - 40 y^3 + 29 y^2 + 82 y - 7 <= 0] "300 300 -4 4 -4 4" '(sset true) '(ord (y z)))

# the second part
(plot2d [z^2 + 2 y^2 - 1 = 0 /\ z^2 + 2 y z + 2 z + y^2 + 10 y - 7 <= 0] "300 300 -4 4 -4 4" '(sset true) '(ord (y z)))

(plot2d [z^2 + 2 y^2 - 1 /= 0 /\ z^6 + 2 y z^5 + 2 z^5 + 5 y^2 z^4 + 10 y z^4 - 9 z^4 + 8 y^3 z^3 + 8 y^2 z^3 - 4 y z^3 - 4 z^3 + 8 y^4 z^2 + 40 y^3 z^2 - 34 y^2 z^2 - 20 y z^2 + 15 z^2
 + 8 y^5 z + 8 y^4 z - 8 y^3 z - 8 y^2 z + 2 y z + 2 z + 4 y^6 + 40 y^5 - 32 y^4 - 40 y^3 + 29 y^2 + 82 y - 7 <= 0  \/ z^2 + 2 y^2 - 1 = 0 /\ z^2 + 2 y z + 2 z + y^2 + 10 y - 7 <= 0] "300 300 -4 4 -4 4" '(sset true) '(ord (y z)))

# ex ex1.svg
(plot2d [z^2 + 2 y^2 - 1 /= 0 /\ z^6 + 2 y z^5 + 2 z^5 + 5 y^2 z^4 + 10 y z^4 - 9 z^4 + 8 y^3 z^3 + 8 y^2 z^3 - 4 y z^3 - 4 z^3 + 8 y^4 z^2 + 40 y^3 z^2 - 34 y^2 z^2 - 20 y z^2 + 15 z^2 + 8 y^5 z + 8 y^4 z - 8 y^3 z - 8 y^2 z + 2 y z + 2 z + 4 y^6 + 40 y^5 - 32 y^4 - 40 y^3 + 29 y^2 + 82 y - 7 <= 0  \/ z^2 + 2 y^2 - 1 = 0 /\ z^2 + 2 y z + 2 z + y^2 + 10 y - 7 <= 0] "300 300 -4.5 4.5 -4.5 4.5 ex1.svg" '(sset true) '(ord (y z)))

# ex ex1a.svg (just the first part)
(plot2d [z^2 + 2 y^2 - 1 /= 0 /\ z^6 + 2 y z^5 + 2 z^5 + 5 y^2 z^4 + 10 y z^4 - 9 z^4 + 8 y^3 z^3 + 8 y^2 z^3 - 4 y z^3 - 4 z^3 + 8 y^4 z^2 + 40 y^3 z^2 - 34 y^2 z^2 - 20 y z^2 + 15 z^2 + 8 y^5 z + 8 y^4 z - 8 y^3 z - 8 y^2 z + 2 y z + 2 z + 4 y^6 + 40 y^5 - 32 y^4 - 40 y^3 + 29 y^2 + 82 y - 7 <= 0] "300 300 -4.5 4.5 -4.5 4.5 ex1a.svg" '(sset true) '(ord (y z)))


inkscape --file=image.svg --without-gui --export-pdf=image.pdf

inkscape --file=ex1.svg --without-gui --export-pdf=ex1.pdf
inkscape --file=ex1a.svg --without-gui --export-pdf=ex1a.pdf


==> ex3 <==
Good example!


[
rewritten for
all z[ 1/(x z^2 + y z + x) < 1 ]
]
(x,y,z)
2
(A z)[
[ [x /= 0 \/ y /= 0] /\
   [ x z^2 + y z + x = 0 \/ (x z^2 + y z + x) < (x z^2 + y z + x)^2 ]
]
\/
[z^2 < (x + y) ]
].
go
go
go
d-2d-cad E -2 2 -2 2 500 500 0.1


[
"bad" rewritingx for
all z[ 1/(x z^2 + y z + x) < 1 ]
]
(x,y,z)
2
(A z)[
[
[ x z^2 + y z + x = 0 \/ (x z^2 + y z + x) < (x z^2 + y z + x)^2 ]
]
\/
[z^2 < (x + y) ]
].
go
go
go
d-2d-cad E -2 2 -2 2 500 500 0.1

gives true at (x,y) = (0,0)

[
"worse" rewriting for
all z[ 1/(x z^2 + y z + x) < 1 ]
]
(x,y,z)
2
(A z)[
[
[ x z^2 + y z + x = 0 /\ (x z^2 + y z + x) < (x z^2 + y z + x)^2 ]
]
\/
[z^2 < (x + y) ]
].
go
go
go

Gives false everywhere

[
remove denominators without worrying about the possiblity
of denominators being zero
all z[ 1/(x z^2 + y z + x) < 1 ]
]
(x,y,z)
2
(A z)[
[
 (x z^2 + y z + x) < (x z^2 + y z + x)^2 
]
\/
[z^2 < (x + y) ]
].
go
go
go

Gives false on the boundary of the left-most component, which
should be true because the only "bad z" value is where the denominator
vanishes, which we don't want to count as a "bad" value for the "forall".



==> ex4 <==
## Example 1 - interesting example to apply translate(F,A) to
[ all a,b[ex x[ x - div(1,a x + b div(1,b+1)) = 0 ] ] ]

# Solution (correct!)
[all a,b[ex x[b + 1 = 0 \/ [x^2 a b + x b - b + x^2 a - 1 = 0 /\ x a b + b + x a /= 0] \/ [b = 0 /\ a = 0]]]]

# Incorrect solution that I had worked out by hand and messed up on!
[ all a,b[ex x[ b + 1 = 0 \/ a = 0 /\ b = 0 \/ [ (b+1) a x + b /= 0 /\ (b + 1) (a x^2 + b x - 1) = 0 ] ] ] ]


## Example 2  - expand example to a formula ... note: this is not fair-SAT! because at (a,b) = (-1/4,1) the only x that makes (a x^2 + b x - 1) = 0 also makes the denominator zero!
[ all a,b[ex x[ b^2 + 4 a >= 0 ==> x - div(1,a x + b div(1,b+1)) = 0 ] ] ]



[ all a,b[ ex x [ b^2 + 4 a >= 0 ==> [ b + 1 = 0 \/ a = 0 /\ b = 0 \/ [ (b+1) a x + b /= 0 /\ (b + 1) (a x^2 + b x - 1) = 0 ] ] ] ] ]


## Example 3 - this is fair-SAT!
[ all a,b[ex x[ b /= 1 /\ b^2 + 4 a >= 0 ==> x - div(1,a x + b div(1,b+1)) = 0 ] ] ]

[ all a,b[ ex x [ b /= 1 /\ b^2 + 4 a >= 0 ==> [ b + 1 = 0 \/ a = 0 /\ b = 0 \/ [ (b+1) a x + b /= 0 /\ (b + 1) (a x^2 + b x - 1) = 0 ] ] ] ] ]


## Example 4 - this has free variable r.  It is fair-SAT for all r s.t. r <= 3/4.
[ all a,b[ex x[ b + a < r /\ b^2 + 4 a >= 0 ==> x - div(1,a x + b div(1,b+1)) = 0 ] ] ]

[ all a,b[ ex x [ b + a < r /\ b^2 + 4 a >= 0 ==> [ b + 1 = 0 \/ a = 0 /\ b = 0 \/ [ (b+1) a x + b /= 0 /\ (b + 1) (a x^2 + b x - 1) = 0 ] ] ] ] ]




